Verifying Safety of Functional Programs with Rosette/Unbound

The goal of unbounded program verification is to discover an inductive invariant that safely over-approximates all possible program behaviors. Functional languages featuring higher order and recursive functions become more popular due to the domain-specific needs of big data analytics, web, and security. We present Rosette/Unbound, the first program verifier for Racket exploiting the automated constrained Horn solver on its backend. One of the key features of Rosette/Unbound is the ability to synchronize recursive computations over the same inputs allowing to verify programs that iterate over unbounded data streams multiple times. Rosette/Unbound is successfully evaluated on a set of non-trivial recursive and higher order functional programs.

==> conclusion.tex <==
\section{Future Work and Conclusion}
\label{sec:concl}

Extracting counter-examples for lists: not an easy task, since we do not operate with lists as a data structure.

Applying with synthesis (integrate with \rosette)

DSLs?
